Understanding the Impact of Domain Term Explanation on Duplicate Bug Report Detection

Duplicate bug reports make up 42% of all reports in bug tracking systems (e.g., Bugzilla), causing significant maintenance overhead. Hence, detecting and resolving duplicate bug reports is essential for effective issue management. Traditional techniques often focus on detecting textually similar duplicates. However, existing literature has shown that up to 23% of the duplicate bug reports are textually dissimilar. Moreover, about 78% of bug reports in open-source projects are very short (e.g., less than 100 words) often containing domain-specific terms or jargon, making the detection of their duplicate bug reports difficult. In this paper, we conduct a large-scale empirical study to investigate whether and how enrichment of bug reports with the explanations of their domain terms or jargon can help improve the detection of duplicate bug reports. We use 92,854 bug reports from three open-source systems, replicate seven existing baseline techniques for duplicate bug report detection, and answer two research questions in this work. We found significant performance gains in the existing techniques when explanations of domain-specific terms or jargon were leveraged to enrich the bug reports. Our findings also suggest that enriching bug reports with such explanations can significantly improve the detection of duplicate bug reports that are textually dissimilar.

==> rebuttal_info.tex <==
Review1-Question1, Review2-Question2: A simple dictionary-based approach might be attractive. Unfortunately, it suffers from vocabulary mismatches between a bug report and the dictionary. The approach cannot explain a domain term if it does not match the entries from the dictionary exactly. Static dictionaries also have fixed, predefined entries with possibly hand-crafted explanations, which might fail to adapt to new or emerging terminologies relevant to bug reports. On the other hand, LLMs (e.g., T5) are pre-trained with vast datasets (e.g., C4 [2]). They can explain partially matched or even lexically unmatched but semantically equivalent domain terms with their strong reasoning capabilities [3]. They also provide context-aware explanations and might be better equipped to tackle the challenges of emerging terminologies due to their large vocabularies, advanced tokenization methods (e.g., Byte-pair encoding [2]), and continuous updates by the community (e.g., HuggingFace).

Review1-Question2: The statistical tests determine if our domain term explanations improve the performance of existing techniques significantly or not. For BM25 and LDA, we used recall rates at k (k=1, 5, 10, 100) as samples, whereas for Siamese CNN and DC-CNN, we used  AUC, Precision, Recall, and F1 scores as samples for our statistical tests. We acknowledge the limitation of using a small sample size (n=4), which may affect the robustness of statistical inferences. However, we also repeated our experiments with recall rates at k from 1 to 100 with 20 samples. We found significant performance improvement for both BM25 (p=6.4E-07) and LDA+GloVe (p=9E-15), with medium (D=0.30) and large (Cohen’s D=1.15) effect sizes, respectively. If accepted, we will report our updated significance statistics in the CR version. 

Review2-Question1: As outlined in Section III-C, we used the authors’ replication packages to avoid any replication-related threats. To our knowledge, no replication package of the reference [9] is publicly available, which prevented us from replicating their work. Besides, our contribution lies in explaining the domain-specific terms and measuring their impacts on duplicate bug report detection. Since the existing work [9] only extracts the domain terms and does not explain them, our work is complementary to theirs and thus could also benefit theirs.

Review2-Question3, Review2-Comment3: Our study advances the state-of-the-art in duplicate bug report detection in two ways. First, existing techniques for duplicate bug report detection suffer from low performance when duplicate bug reports use lexically dissimilar terminologies (RQ2). Our explanations of domain-specific terms equip existing techniques with more contextual information to perform significantly better in detecting duplicate bug reports, as shown by our experiments (Tables VIII, IX). Second, bug reports often suffer from poor quality or lack of interpretability, making their comprehension difficult. Our work explains their domain terms and provides more contexts, which could help developers comprehend the bug reports and locate duplicates easily. Furthermore, our idea of explaining domain terms has broader applications beyond duplicate bug detection. For example, in code summarization and search, explanations of domain-specific identifier names can help developers navigate unfamiliar codebases or legacy systems. Similarly, our explanations can improve bug understanding or reproduction by familiarising novice developers with specific APIs or domains.

Review3-Question1, Review1-Concern3: We collected the textually similar and dissimilar subsets from the benchmark dataset of Jahan et al. [1]. First, they collected duplicate bug reports from three open-source repositories – Eclipse, Mozilla, and Firefox – with duplicate ratios of 6.60%, 20.53%, and 10.56%, respectively.  Second, they calculated the cosine similarity score for each pair of duplicate bug reports using N-grams (n = 1, 2, 3). Third, they analysed the distribution of the similarity scores and identified the median and quartiles.  Finally, they marked the pairs with scores below the 25th percentile as textually dissimilar and those above the 75th percentile as textually similar duplicates. To avoid noise, they identified the bug report pairs consistently found to be similar or dissimilar across all three N-gram trials and kept them in two distinct subsets for their analysis [1].

Review3-Question2: The lower performances of SiameseCNN and DC-CNN in Table IX could be explained by the smaller sizes of their datasets. Deep learning models require large datasets to learn robust features and to perform well. Smaller datasets (e.g., textually similar, textually dissimilar) limit the models’s ability to capture complex semantic relationships. However, despite these challenges, our study shows that the enrichment of bug reports with domain-term explanations consistently improved the models’ performance across all metrics (RQ1, RQ2).

Comments

Review3-Concern1: In this work, we did not assess the impact of explanations from different sources, individually or in combination, but this presents an excellent opportunity for future work. We believe that the explanations might be complementary given that our sources target different aspects of a programming domain (e.g., API documentation, question answering, code examples).

Review2-Concern1: While we acknowledge that PR-AUC is often preferred for imbalanced datasets, we chose to maintain ROC-AUC as an evaluation metric since the original work [1] adopted that metric for their experiment. We wanted to replicate the existing work reliably.

Review2-Concern2: In this work, we demonstrate the impact of domain term explanations on duplicate bug report detection. However, we also evaluated the generated explanations against the ground truth explanations, which were not included in the paper due to space constraints. We acknowledge that including these evaluations would strengthen our findings. If accepted, we would add a discussion in the CR copy.


Review1-Concern1: API documentation and Glossary might contain duplicate entries that should be consolidated. Since both are managed by the same organisation – Oracle [4], [10], keeping one source of explanation per term might be sufficient.

% incorporated
Review1-Concern2: We adopted the regularization parameters from T5's original architecture [2] at HuggingFace, which were found to be effective across various natural language tasks [11], [12], [13].


Review1-Concern4: Performance Metrics were selected based on the underlying methodologies of the selected baselines – Information Retrieval, Topic Modelling, and Deep Learning. They are also widely used in the relevant literature [5 - 8].




% meta review info

Meta-Review
Thank you to the authors for their submission to MSR 2025. The reviewers appreciated the focus on an important and timely topic and found the concept of leveraging explanations to enhance bug report detection performance interesting. However, after careful consideration, the reviewers could not recommend the current version of the paper for acceptance due to the following significant concerns:
The paper does not evaluate its approach against established state-of-the-art models in the field, such as BERT, for bug report detection. This omission makes it difficult to contextualize the contribution and understand how the proposed approach advances the current state of the art.
The reported performance gains are quite small, which raises questions about the practical impact of the approach. Stronger results or additional justifications for the significance of these improvements should be provided to demonstrate the value of this contribution.
The statistical tests used to validate the findings are not clearly described, making it challenging to assess their correctness or the validity of the reported results. Clear and rigorous reporting of statistical methodologies is critical for the credibility of empirical studies.
We encourage the authors to continue refining this work and hope they will incorporate the reviewers' feedback to strengthen the quality of the work.


Reviewer 1 : Questions for the author's response
Q1: Why not use a simpler version of the approach with a dictionary of definitions instead of an LLM?
Q2: What are the samples used in the statistical tests? Did you subset the data?
Comments on the author's response
I am still concerned with the absence of a baseline, but I appreciate the proposal to improve the statistical tests. However, it is not very clear to me how they propose to solve the issue. It would be reasonable to subset the dataset, I do not understand why they used recall at k. An explicit definition of null and alternative hypotheses could lead to better clarity, and ensure soundness.

Reviewer 2 : Questions for the author's response
Why was the relevant model in Reference [9] not included in the comparison?
What is the advantage of using a pre-trained T5 model for generating explanations compared to using the pairs of domain-specific terms and explanations directly?
How can the study advance the state-of-the-art(s) of duplicate bug report detection when the performance improvements are quite small and sometimes not even significant?

Comments on the author's response
Thank you to the authors for answering my questions. Please find below my comments on the authors' answers to each of the questions.
For Q1, the authors mentioned they could not replicate Reference [9]. However, this work was mainly based on the BERT model, which is readily available. The authors could have tried the BERT model and reported the findings to improve the relevance of the findings to the latest advances in the field.
For Q2, the authors' response makes sense to me.
For Q3, the authors did not directly address the concern about the insignificant performance improvements using the proposed approach. Thus, my concern still remains that the findings will be unlikely to change the latest practices of this task moving forward.
Overall, I was not fully satisfied with the rebuttal, so I decided to keep my original score.


Reviewer 3 : Questions for the author's response
The make or break question to me is: what was the methodology for the construction of the groups in RQ2?
Another important question is: how do the authors explain the obtained results for SiameseCNN and DC-CNN in Table IX and how worse they were, compared to the results in Table VII?
Comments on the author's response
I thank the authors for the responses to my questions. The explanation about the methodology for the construction of the groups is an improvement over the current status of the paper.
As for my second question, I don't think the authors really responded it. Furthermore, the point that I raised in the review about BM25 and LDA+GloV was not addressed in the authors' response, about cases where there was a lot of room for improvement improving only a little.
In the light of these considerations, I am maintaining my recommendation of Weak Reject.

